FRAPPE: Full Input, Residual Output Autoencoding with Projection Pursuit Encoder

Media compression standards have reached a plateau in terms of the rate-distortion-complexity trade-off, limiting the ability to offload expensive AI perception to the cloud in applications like robotics, wearables, and remote sensing. DNN-based codecs improve compression efficiency, but at a cost: they cannot easily adapt to large changes in available bitrate, and real-time encoding requires expensive, power-hungry GPUs that prohibit use on low-cost or resource-constrained platforms. To address these limitations, we propose a novel autoencoding framework (FRAPPE) that uses the Full input to predict the Residual output via a Projection Pursuit Encoder. FRAPPE's encoding objective naturally sorts latent channels by importance, allowing zero-overhead variable-rate coding. Unlike RNN-based learned codecs, whose encoder consumes the previous reconstruction's residual, or RVQ-style codecs, whose codebooks must be applied sequentially, FRAPPE's analysis path is an embarrassingly parallel DAG of independent input projections. Using FRAPPE, we build a variable-rate RGB image codec (FRAPPE-Image), and evaluate its rate-distortion-complexity trade-off against standard image codecs. At high compression ratios (approx. 0.1 bpp) FRAPPE-Image provides higher perceptual quality than AVIF with 47 times faster encoding, making it capable of real-time 1080p, 30fps CPU-only encoding. Our code and pre-trained models are available: https://github.com/UT-SysML/FRAPPE .

==> figures/rd_throughput_table.tex <==
\begin{tabular}{llrrrrr}
\toprule
Codec & Setting & bpp & PSNR (dB) & SSIM & DISTS (dB) & Throughput (MPx/s) \\
\midrule
JPEG & $q=1$ & 0.17309 & 21.48 & 0.6152 & 4.56 & 543.97 \\
JPEG & $q=5$ & 0.22115 & 23.85 & 0.7326 & 5.80 & 530.25 \\
JPEG & $q=10$ & 0.32659 & 26.67 & 0.8419 & 7.74 & 529.90 \\
JPEG & $q=15$ & 0.42310 & 28.14 & 0.8883 & 9.16 & 501.51 \\
JPEG & $q=20$ & 0.50827 & 29.14 & 0.9139 & 10.25 & 469.02 \\
JPEG & $q=25$ & 0.58768 & 29.89 & 0.9294 & 11.29 & 487.97 \\
JPEG & $q=30$ & 0.65979 & 30.49 & 0.9400 & 11.98 & 475.52 \\
JPEG & $q=35$ & 0.72857 & 31.01 & 0.9478 & 12.73 & 479.66 \\
JPEG & $q=40$ & 0.78557 & 31.42 & 0.9530 & 13.25 & 469.90 \\
JPEG & $q=45$ & 0.84921 & 31.82 & 0.9577 & 13.84 & 463.71 \\
JPEG & $q=50$ & 0.90552 & 32.17 & 0.9613 & 14.32 & 455.88 \\
JPEG & $q=55$ & 0.96365 & 32.52 & 0.9643 & 14.69 & 436.14 \\
JPEG & $q=60$ & 1.03659 & 32.91 & 0.9675 & 15.18 & 444.06 \\
JPEG & $q=65$ & 1.12648 & 33.36 & 0.9707 & 15.78 & 435.98 \\
JPEG & $q=70$ & 1.23876 & 33.92 & 0.9741 & 16.59 & 427.69 \\
JPEG & $q=75$ & 1.36760 & 34.52 & 0.9772 & 17.25 & 407.08 \\
JPEG & $q=80$ & 1.57024 & 35.37 & 0.9807 & 18.33 & 398.82 \\
JPEG & $q=85$ & 1.85652 & 36.46 & 0.9842 & 19.75 & 384.55 \\
JPEG & $q=90$ & 2.34632 & 38.03 & 0.9880 & 21.29 & 354.31 \\
JPEG & $q=95$ & 3.39192 & 40.56 & 0.9919 & 23.44 & 307.11 \\
JPEG & $q=100$ & 6.78674 & 44.86 & 0.9973 & 25.75 & 212.35 \\
JPEG XL & $q=5$ & 0.14307 & 25.81 & 0.7859 & 7.15 & 3.17 \\
JPEG XL & $q=10$ & 0.17342 & 26.63 & 0.8173 & 7.69 & 3.29 \\
JPEG XL & $q=20$ & 0.29262 & 28.70 & 0.8874 & 9.64 & 3.63 \\
JPEG XL & $q=30$ & 0.39710 & 30.04 & 0.9201 & 11.14 & 3.65 \\
JPEG XL & $q=50$ & 0.51894 & 31.31 & 0.9419 & 12.56 & 3.60 \\
JPEG XL & $q=70$ & 0.81463 & 33.56 & 0.9651 & 14.96 & 4.14 \\
JPEG XL & $q=85$ & 1.42035 & 36.85 & 0.9813 & 18.47 & 4.28 \\
JPEG XL & $q=95$ & 2.84492 & 41.44 & 0.9921 & 24.40 & 6.41 \\
AVIF & $q=1$ & 0.06814 & 25.60 & 0.7727 & 6.60 & 6.04 \\
AVIF & $q=5$ & 0.07497 & 25.83 & 0.7865 & 6.81 & 5.78 \\
AVIF & $q=10$ & 0.10373 & 26.78 & 0.8277 & 7.44 & 5.04 \\
AVIF & $q=15$ & 0.12245 & 27.26 & 0.8471 & 7.78 & 4.68 \\
AVIF & $q=20$ & 0.16034 & 28.09 & 0.8754 & 8.59 & 4.96 \\
AVIF & $q=25$ & 0.18705 & 28.59 & 0.8903 & 9.08 & 4.61 \\
AVIF & $q=30$ & 0.24547 & 29.57 & 0.9133 & 9.92 & 3.88 \\
AVIF & $q=35$ & 0.30673 & 30.40 & 0.9303 & 10.88 & 4.01 \\
AVIF & $q=40$ & 0.37911 & 31.25 & 0.9439 & 11.60 & 3.53 \\
AVIF & $q=45$ & 0.49205 & 32.45 & 0.9573 & 12.73 & 3.82 \\
AVIF & $q=50$ & 0.60038 & 33.39 & 0.9658 & 13.73 & 3.33 \\
AVIF & $q=55$ & 0.71940 & 34.31 & 0.9721 & 14.69 & 3.02 \\
AVIF & $q=60$ & 0.88589 & 35.45 & 0.9779 & 15.67 & 2.71 \\
AVIF & $q=65$ & 1.00195 & 36.17 & 0.9807 & 16.52 & 2.89 \\
AVIF & $q=70$ & 1.23831 & 37.49 & 0.9843 & 17.50 & 2.82 \\
AVIF & $q=75$ & 1.41952 & 38.29 & 0.9867 & 18.58 & 2.64 \\
AVIF & $q=80$ & 1.66593 & 39.18 & 0.9890 & 19.80 & 2.45 \\
AVIF & $q=85$ & 1.90300 & 39.93 & 0.9905 & 20.64 & 2.43 \\
AVIF & $q=90$ & 2.47039 & 41.26 & 0.9922 & 22.02 & 2.19 \\
AVIF & $q=95$ & 3.36300 & 42.61 & 0.9943 & 23.18 & 1.99 \\
AVIF & $q=100$ & 5.82183 & 44.43 & 0.9976 & 24.85 & 1.97 \\
mbt2018 & $q=1$ & 0.11021 & 28.12 & 0.8556 & 7.73 & 0.17 \\
mbt2018 & $q=2$ & 0.19508 & 29.64 & 0.8934 & 8.57 & 0.17 \\
mbt2018 & $q=3$ & 0.28821 & 31.39 & 0.9301 & 10.05 & 0.17 \\
mbt2018 & $q=4$ & 0.43015 & 33.19 & 0.9543 & 11.35 & 0.17 \\
mbt2018 & $q=5$ & 0.63418 & 35.14 & 0.9694 & 12.88 & 0.16 \\
mbt2018 & $q=6$ & 0.88206 & 37.07 & 0.9800 & 14.87 & 0.17 \\
mbt2018 & $q=7$ & 1.19641 & 38.98 & 0.9867 & 17.15 & 0.16 \\
mbt2018 & $q=8$ & 1.58371 & 40.67 & 0.9912 & 19.44 & 0.16 \\
WaLLoC & $q=1$ & 0.00968 & 20.43 & 0.5165 & 4.05 & 74.83 \\
WaLLoC & $q=2$ & 0.02035 & 21.93 & 0.5866 & 4.73 & 74.02 \\
WaLLoC & $q=4$ & 0.03244 & 22.79 & 0.6373 & 5.21 & 66.27 \\
WaLLoC & $q=8$ & 0.06279 & 24.02 & 0.7174 & 6.12 & 45.45 \\
WaLLoC & $q=16$ & 0.11444 & 25.22 & 0.7906 & 7.20 & 30.37 \\
WaLLoC & $q=25$ & 0.17037 & 26.11 & 0.8391 & 8.29 & 24.64 \\
WaLLoC & $q=36$ & 0.23783 & 26.95 & 0.8711 & 9.14 & 19.63 \\
WaLLoC & $q=56$ & 0.35890 & 28.29 & 0.9100 & 10.71 & 20.83 \\
WaLLoC & $q=80$ & 0.50761 & 29.60 & 0.9355 & 12.00 & 14.66 \\
WaLLoC & $q=100$ & 0.61707 & 30.56 & 0.9501 & 13.26 & 14.19 \\
LiVeAction & $q=4$ & 0.03406 & 22.98 & 0.6376 & 5.13 & 1.90 \\
LiVeAction & $q=9$ & 0.07338 & 24.36 & 0.7309 & 6.25 & 1.72 \\
LiVeAction & $q=16$ & 0.12398 & 25.37 & 0.7955 & 7.25 & 1.81 \\
LiVeAction & $q=25$ & 0.18668 & 26.31 & 0.8461 & 8.35 & 1.93 \\
LiVeAction & $q=36$ & 0.26190 & 27.21 & 0.8793 & 9.25 & 1.54 \\
LiVeAction & $q=49$ & 0.34935 & 28.15 & 0.9072 & 10.30 & 1.73 \\
LiVeAction & $q=64$ & 0.45422 & 29.17 & 0.9295 & 11.38 & 1.89 \\
LiVeAction & $q=81$ & 0.56666 & 30.13 & 0.9452 & 12.46 & 1.63 \\
LiVeAction & $q=100$ & 0.69215 & 31.25 & 0.9582 & 13.74 & 1.76 \\
MCUCoder & $q=1$ & 0.08542 & 20.55 & 0.6900 & 5.21 & 24.29 \\
MCUCoder & $q=2$ & 0.15461 & 23.69 & 0.7784 & 6.70 & 22.69 \\
MCUCoder & $q=3$ & 0.21980 & 25.04 & 0.8168 & 7.67 & 21.08 \\
MCUCoder & $q=4$ & 0.27952 & 25.66 & 0.8409 & 8.23 & 20.24 \\
MCUCoder & $q=5$ & 0.33768 & 26.12 & 0.8633 & 8.80 & 19.17 \\
MCUCoder & $q=6$ & 0.39355 & 26.56 & 0.8717 & 9.30 & 18.17 \\
MCUCoder & $q=7$ & 0.44407 & 26.83 & 0.8815 & 9.69 & 17.35 \\
MCUCoder & $q=8$ & 0.49997 & 27.09 & 0.8907 & 10.05 & 16.30 \\
MCUCoder & $q=9$ & 0.55529 & 27.32 & 0.8982 & 10.37 & 15.90 \\
MCUCoder & $q=10$ & 0.60788 & 27.53 & 0.9044 & 10.57 & 15.22 \\
MCUCoder & $q=11$ & 0.66242 & 27.71 & 0.9090 & 10.81 & 14.62 \\
MCUCoder & $q=12$ & 0.71329 & 27.84 & 0.9129 & 10.95 & 14.13 \\
FRAPPE & $n=1$ & 0.00424 & 18.54 & 0.4942 & 3.16 & 887.27 \\
FRAPPE & $n=2$ & 0.00639 & 20.30 & 0.5254 & 3.75 & 883.77 \\
FRAPPE & $n=3$ & 0.00800 & 21.08 & 0.5455 & 4.17 & 914.94 \\
FRAPPE & $n=4$ & 0.01337 & 21.90 & 0.5870 & 4.66 & 510.48 \\
FRAPPE & $n=5$ & 0.01716 & 22.38 & 0.6165 & 4.96 & 483.56 \\
FRAPPE & $n=6$ & 0.02590 & 23.13 & 0.6647 & 5.57 & 464.29 \\
FRAPPE & $n=7$ & 0.03521 & 23.74 & 0.6939 & 5.96 & 427.58 \\
FRAPPE & $n=8$ & 0.04101 & 24.05 & 0.7159 & 6.24 & 415.67 \\
FRAPPE & $n=9$ & 0.04728 & 24.40 & 0.7294 & 6.50 & 377.87 \\
FRAPPE & $n=10$ & 0.05792 & 24.81 & 0.7520 & 6.75 & 300.73 \\
FRAPPE & $n=11$ & 0.06927 & 25.27 & 0.7738 & 7.07 & 267.54 \\
FRAPPE & $n=12$ & 0.08027 & 25.64 & 0.7881 & 7.34 & 237.35 \\
FRAPPE & $n=13$ & 0.19661 & 27.40 & 0.8740 & 8.91 & 167.76 \\
FRAPPE & $n=14$ & 0.23298 & 27.98 & 0.8909 & 9.27 & 147.96 \\
FRAPPE & $n=15$ & 0.28510 & 28.69 & 0.9067 & 9.86 & 135.11 \\
FRAPPE & $n=16$ & 0.31429 & 29.22 & 0.9108 & 10.03 & 130.73 \\
FRAPPE & $n=17$ & 0.36634 & 29.69 & 0.9209 & 10.37 & 121.67 \\
FRAPPE & $n=18$ & 0.41224 & 29.98 & 0.9267 & 10.66 & 115.51 \\
FRAPPE & $n=19$ & 0.63229 & 30.94 & 0.9413 & 11.41 & 81.26 \\
FRAPPE & $n=20$ & 0.72202 & 31.57 & 0.9431 & 11.57 & 73.60 \\
FRAPPE & $n=21$ & 0.94176 & 32.28 & 0.9546 & 12.26 & 59.57 \\
\bottomrule
\end{tabular}

